Semantic-preserved Communication System for Highly Efficient Speech Transmission

Deep learning (DL) based semantic communication methods have been explored for the efficient transmission of images, text, and speech in recent years. In contrast to traditional wireless communication methods that focus on the transmission of abstract symbols, semantic communication approaches attempt to achieve better transmission efficiency by only sending the semantic-related information of the source data. In this paper, we consider semantic-oriented speech transmission which transmits only the semantic-relevant information over the channel for the speech recognition task, and a compact additional set of semantic-irrelevant information for the speech reconstruction task. We propose a novel end-to-end DL-based transceiver which extracts and encodes the semantic information from the input speech spectrums at the transmitter and outputs the corresponding transcriptions from the decoded semantic information at the receiver. For the speech to speech transmission, we further include a CTC alignment module that extracts a small number of additional semantic-irrelevant but speech-related information for the better reconstruction of the original speech signals at the receiver. The simulation results confirm that our proposed method outperforms current methods in terms of the accuracy of the predicted text for the speech to text transmission and the quality of the recovered speech signals for the speech to speech transmission, and significantly improves transmission efficiency. More specifically, the proposed method only sends 16% of the amount of the transmitted symbols required by the existing methods while achieving about 10% reduction in WER for the speech to text transmission. For the speech to speech transmission, it results in an even more remarkable improvement in terms of transmission efficiency with only 0.2% of the amount of the transmitted symbols required by the existing method.

==> related_work.tex <==
\section{Related Work}
This section first introduces the related work on semantic communication systems to demonstrate the current method to extract semantic information. Then, we discuss the modern speech to text and text to speech models to address the alignment method of sequential time series data to further compress the semantic features.

%\subsection{End-to-End Communication Systems}
%The DL-enabled E2E communication systems have achieved extremely competitive block-error rate (BLER) performance in comparison to the traditional block-wise communication systems in various scenarios\cite{o2017introduction}. In addition, it has shown great potentials in processing complicated communication tasks. For examples, the E2E learning has been employed in orthogonal frequency division multiplexing (OFDM) systems\cite{kim2017novel,felix2018ofdm}, as well as in multiple-input multiple-output (MIMO) systems\cite{o2017physical,he2020model}. Besides, channel estimation is a challenging problem in the DL-enabled E2E systems. In\cite{aoudia2019model}, reinforcement learning (RL) has been adopted to estimate the channel state information (CSI) through treating the channel layer and the receiver as the \emph{environment}. However, it requires a reliable channel to feedback the losses from the receiver to the transmitter during the training phase. Another novel channel agnostic solution has been proposed in\cite{ye2020deep}, which replaces the realistic channel with a deep neural network (DNN) by exploiting a conditional generative adversarial network (GAN).

%Due to the complexity of NN training, a system with high training efficiency and low energy consumption is more than desired to make the E2E system applicable in practice. Transfer learning is a promising technology for adapting E2E communication systems to cope with the uncontrollable and unpredictable channel environments by training them over a statistical channel model\cite{pan2009survey}. Another appealing solution is to obtain a trained model yielding expected performance via the stochastic gradient descent (SGD) with a small number of iterations. Particularly, based on model-agnostic meta-learning (MAML), an E2E communication system has been developed in\cite{park2020meta}, which finds the initial NN parameters to achieve fast convergence for various channel conditions.

%\subsection{Semantic Communications}
%An initial research on semantic communication systems for text information was developed\cite{guler2018semantic}, which mitigates the semantic error by integrating the semantic inference and the physical layer communications to optimize the whole transceiver. However, such a text-based semantic communication system only measures the semantic error at the word level instead of the sentence level. Thus, a further investigation on semantic text transmission, named DeepSC, has been developed\cite{9398576} to deal with the semantic error at the sentence level with various length. Powered by the Transformer\cite{10.5555/3295222.3295349}, the semantic encoder and the channel encoder are co-designed to minimize the semantic error and to improve the system capacity. Moreover, the increasing deployment of smart IoT applications requires IoT devices to be capable of dealing with more complicated tasks, which runs counter to the limited computing capability of IoT devices. Inspired by this, a lite distributed semantic communication system for text transmission, named L-DeepSC\cite{xie2020lite}, has been further proposed to address the challenge of IoT devices by pruning and quantizing NN parameters. By doing so, the size of the trained model as well as the communication cost between the IoT devices and the server are reduced significantly, which makes it more suitable for IoT applications.

%In semantic communications for image information, a DL-enabled semantic communication system has been developed\cite{bourtsoulatze2019deep}, which employs a convolutional neural network (CNN) at the transmitter to jointly design the source-channel coding. Besides, an image transmission system has been investigated to improve the accuracy of image reconstruction\cite{kurka2020deepjscc}, which backpropagates the channel output in order to generate a weight vector to the NN at the transmitter. In addition to perform the typical image reconstruction, more intelligent tasks have been considered. Particularly, an application based on a joint source-channel coding (JSCC) model to retrieve image has been proposed\cite{jankowski2020wireless}, which aims to reduce the transmission latency for IoT devices by achieving retrieval-oriented image compression. Besides, a joint image transmission-recognition system has been developed\cite{lee2019deep} for IoT applications, which has the superior recognition accuracy than the traditional approaches but requires the affordable computation resource. Moreover, by exploiting NN compression techniques, a deep JSCC\cite{jankowski2020joint} has been developed to perform image classification at the edge sever, which facilitates the IoT devices to process images with low computational complexity and to reduce the required transmission bandwidth. Note that the concept of semantic communications was not clearly stated by the authors in the aforementioned work on image transmission. However, we treat them as the pioneering works in the area as they share the spirit of semantic communications by extracting and transmitting the relevant information from the source for serving the transmission goals at the receiver.


% # 语义通信的发展历程和现状
\subsection{Semantic Communication}
The idea of using semantic communication has a relative long history, which has been proposed by Weaver at the beginning of modern communication\cite{shannon1949mathematical}. Following this preliminary work, Carnap and Bar-hillel \cite{carnap1952outline} give an information theoretic definition of semantic information, which is further investigated in \cite{bao2011towards}. A semantic aware data compression method has been proposed in \cite{basu2014preserving} by leveraging a shared knowledge base. However, before the boom of deep learning, there has not been an effective way to actually perform semantic communication of content.

The DL-enabled semantic communication systems have achieved extremely competitive accuracy performance compared to the traditional block-wise communication systems in various scenarios. In addition, it has shown great potential in complicated communication conditions, especially under low SNR conditions. A CNN model was presented in \cite{bourtsoulatze2019deep} to enable joint source and channel coding (JSCC) for wireless image transmission, which can recover images under limited bandwidth and low SNR conditions, and achieves efficient image transmission. \cite{kurka2021bandwidth} designed a deep JSCC system for wireless image transmission with multiple refinement Layers of different compression rates to learn the layered representation of image transmission, which can achieve good accuracy under different channel conditions.
A deep learning-based semantic communication system has been developed for efficient and robust transmission of text in \cite{qin1}, the deep learning model of which is then further compressed to be able to work on IoT devices \cite{xie2020lite}. \cite{xie2021task} and \cite{xie2021task1} designed semantic communication systems that are capable of multimodal data transmission for tasks, such as visual question answering. A semantic system was developed for video wireless transmission, which use reinforcement learning to optimize bandwidth allocation and choose adaptive GoP sizes  \cite{tung2021deepwive}.
\subsection{Speech to Text and Text to Speech}
Speech to text method, also known as speech recognition, is an end-to-end model to transform the input speech to its transcription with the help of a deep learning method. The most complicated mission of an end-to-end speech to text model is to map a sequence of input acoustic features into a sequence of grapheme or words. This mapping mission is also called alignment. Now there are two main structures for the alignment: the attention model\cite{chan2016listen}\cite{chorowski2015attention} and CTC\cite{pmlr-v48-amodei16}. Attention-based methods use an attention mechanism to perform alignment between acoustic frames and recognized text, and CTC uses Markov assumptions to compute the conditional distribution over all the input frames.


Text to speech method, also known as speech synthesis, can be used together with Generative Adversarial Networks(GAN) to transform text to the corresponding speech. The transformer-based sequence to sequence models are often used to generate the spectrum of speech and the GANs are used to recover the speech signal from the spectrum. The state-of-art model is Fastspeech2\cite{ren2020fastspeech}, which composes mainly of two feed-forward Transformer stacks and Variance adaptor to predict the duration, pitch and power of speech.
